CC-Light eQASM Architecture Specification

This document is the specification of the CC-Light instantiation of executable QASM (eQASM), a quantum instruction set architecture (QISA) developed in QuTech targeting to control a seven-qubit superconducting quantum processor. This document can serve as a reference manual for low-level programmers, compiler backend developers, and microarchitecture implementers of eQASM. The design of CC-Light eQASM is under the Apache 2.0 License.

==> ex_code/cs.tex <==
         Condition  OpTypeLeft  CW_Left  OpTypeRight  CW_Right
     0:      0          0           0          0          0    
     48:     2          1           0          0          0
     55:     2          1           7          0          0
     49:     2          1           1          0          0
     51:     2          1           3          0          0
     53:     2          1           5          0          0
     50:     2          1           2          0          0
     52:     2          1           4          0          0
     54:     2          1           6          0          0
     56:     2          1           8          0          0
     40:     1          1           0          0          0
     47:     1          1           7          0          0
     41:     1          1           1          0          0
     43:     1          1           3          0          0
     45:     1          1           5          0          0
     42:     1          1           2          0          0
     44:     1          1           4          0          0
     46:     1          1           6          0          0
     8:      0          1           0          0          0
     9:      0          1           1          0          0
     10:     0          1           2          0          0
     11:     0          1           3          0          0
     12:     0          1           4          0          0
     13:     0          1           5          0          0
     14:     0          1           6          0          0
     15:     0          1           7          0          0
     16:     0          1           8          0          0
     17:     0          1           9          0          0
     18:     0          1          10          0          0
     19:     0          1          11          0          0
     20:     0          1          12          0          0
     21:     0          1          13          0          0
     22:     0          1          14          0          0
     23:     0          1          15          0          0
     24:     0          1          16          0          0
     25:     0          1          17          0          0
     26:     0          1          18          0          0
     27:     0          1          19          0          0
     28:     0          1          20          0          0
     29:     0          1          21          0          0
     30:     0          1          22          0          0
     31:     0          1          23          0          0
     32:     0          1          24          0          0
     33:     0          1          25          0          0
     34:     0          1          26          0          0
     35:     0          1          27          0          0
     36:     0          1          28          0          0
     37:     0          1          29          0          0
     38:     0          1          30          0          0
     39:     0          1          31          0          0
     129:    0          2           1          2          1
     128:    0          2           0          2          0
     130:    0          2           2          2          2
     131:    0          2           3          2          3
     132:    0          2           4          2          4
     133:    0          2           5          2          5
     134:    0          2           6          2          6
     135:    0          2           7          2          7
     4:      0          3           0          0          0
     2:      0          0           0          0          0


==> utils/alias_table <==

 \\ \hline
\lstinline!BRA addr!            & \lstinline!BR always, addr!                         & PC = addr << 2 \\ \hline
\lstinline!BRN addr!            & \lstinline!BR never, addr!                          & No operation \\ \hline
\lstinline!BEQ Rs, Rt, addr!    & \lstinline!CMP Rs, Rt!          \lstinline!BR eq, addr!         &  \\ \hline
\lstinline!BNE Rs, Rt, addr!    & \lstinline!CMP Rs, Rt!          \lstinline!BR ne, addr!         &  \\ \hline
\lstinline!BLT Rs, Rt, addr!    & \lstinline!CMP Rs, Rt!          \lstinline!BR lt, addr!         &  \\ \hline
\lstinline!BLE Rs, Rt, addr!    & \lstinline!CMP Rs, Rt!          \lstinline!BR le, addr!         &  \\ \hline
\lstinline!BGT Rs, Rt, addr!    & \lstinline!CMP Rs, Rt!          \lstinline!BR gt, addr!         &  \\ \hline
\lstinline!BGE Rs, Rt, addr!    & \lstinline!CMP Rs, Rt!          \lstinline!BR ge, addr!         &  \\ \hline
\lstinline!BLTU Rs, Rt, addr!   & \lstinline!CMP Rs, Rt!          \lstinline!BR ltu, addr!        &  \\ \hline
\lstinline!BLEU Rs, Rt, addr!   & \lstinline!CMP Rs, Rt!          \lstinline!BR leu, addr!        &  \\ \hline
\lstinline!BGTU Rs, Rt, addr!   & \lstinline!CMP Rs, Rt!          \lstinline!BR gtu, addr!        &  \\ \hline
\lstinline!BGEU Rs, Rt, addr!   & \lstinline!CMP Rs, Rt!          \lstinline!BR geu, addr!        &  \\ \hline
\lstinline!MOV Rd, Rs!          & \lstinline!LDI Rd, 0!           \lstinline!ADD Rd, Rs, Rd!      & Rd = R[rs] \\ \hline
\lstinline!SHL1 Rd, Rs!         & \lstinline!ADD Rd, Rs, Rs!                          & Rd = R[rs] << 1 \\ \hline
\lstinline!MULT2 Rd, Rs!        & \lstinline!ADD Rd, Rs, Rs!                          & Rd = R[rs] * 2 \\ \hline
\lstinline!NAND Rd, Rs, Rt!     & \lstinline!AND Rd, Rs, Rt!      NOT Rd, Rd          & Rd = ~(R[rs] & R[rt]) \\ \hline
\lstinline!NOR Rd, Rs, Rt!      & \lstinline!OR  Rd, Rs, Rt!      NOT Rd, Rd          & Rd = ~(R[rs] | R[rt]) \\ \hline
\lstinline!XNOR Rd, Rs, Rt!     & \lstinline!XOR Rd, Rs, Rt!      NOT Rd, Rd          & Rd = ~(R[rs] ^ R[rt]) \\ \hline

